Momentum and angular correlations in \texorpdfstring{$Z/\gamma$}{Z/gamma}-hadron production in relativistic heavy-ion collisions

We carry out a detailed study of medium modifications on momentum and angular correlations between a large transverse momentum hadron and a $Z/\gamma$ trigger in relativistic heavy-ion collisions within a perturbative QCD parton model improved by the Sudakov resummation technique. The total energy loss of a hard parton propagating inside the medium is employed to modify the fragmentation function, while the medium-induced transverse momentum broadening is included in the resummation approach, and both of them are related to the jet transport parameter and obtained by the high-twist formalism. We obtain good agreements with the existing data on transverse momentum and azimuthal angular correlations for the $Z/\gamma$-hadron pairs in $pp$ and $AA$ collisions, and predict the correlations for the $\gamma$-hadron in central $PbPb$ collisions at 5.02 TeV. The numerical analyses for the $Z/\gamma$-hadron in central $PbPb$ collisions show that the normalized angular distribution is decorrelated due to the medium-induced transverse momentum broadening, however, the angular correlation is enhanced due to the parton energy loss, namely anti-broadening. The observed modification of the angular correlation is a result of the competition between the broadening and the anti-broadening. This work provides a reliable theoretical tool for a comprehensive and precise study of jet quenching in relativistic heavy-ion collisions.

==> ref.tex <==
%\cite{Gyulassy:2004zy}
\bibitem{Gyulassy:2004zy}
M.~Gyulassy and L.~McLerran,
%``New forms of QCD matter discovered at RHIC,''
Nucl. Phys. A \textbf{750}, 30-63 (2005)
doi:10.1016/j.nuclphysa.2004.10.034
[arXiv:nucl-th/0405013 [nucl-th]].
%1277 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Muller:2012zq}
\bibitem{Muller:2012zq}
B.~Muller, J.~Schukraft and B.~Wyslouch,
%``First Results from Pb+Pb collisions at the LHC,''
Ann. Rev. Nucl. Part. Sci. \textbf{62}, 361-386 (2012)
doi:10.1146/annurev-nucl-102711-094910
[arXiv:1202.3233 [hep-ex]].
%485 citations counted in INSPIRE as of 07 Dec 2023

%\cite{Wang:1992qdg}
\bibitem{Wang:1992qdg}
X.~N.~Wang and M.~Gyulassy,
%``Gluon shadowing and jet quenching in A + A collisions at s**(1/2) = 200-GeV,''
Phys. Rev. Lett. \textbf{68}, 1480-1483 (1992)
doi:10.1103/PhysRevLett.68.1480
%970 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Baier:1996kr}
\bibitem{Baier:1996kr}
R.~Baier, Y.~L.~Dokshitzer, A.~H.~Mueller, S.~Peigne and D.~Schiff,
%``Radiative energy loss of high-energy quarks and gluons in a finite volume quark - gluon plasma,''
Nucl. Phys. B \textbf{483}, 291-320 (1997)
doi:10.1016/S0550-3213(96)00553-6
[arXiv:hep-ph/9607355 [hep-ph]].
%1140 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Baier:1996sk}
\bibitem{Baier:1996sk}
R.~Baier, Y.~L.~Dokshitzer, A.~H.~Mueller, S.~Peigne and D.~Schiff,
%``Radiative energy loss and p(T) broadening of high-energy partons in nuclei,''
Nucl. Phys. B \textbf{484}, 265-282 (1997)
doi:10.1016/S0550-3213(96)00581-0
[arXiv:hep-ph/9608322 [hep-ph]].
%1345 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Baier:1998kq}
\bibitem{Baier:1998kq}
R.~Baier, Y.~L.~Dokshitzer, A.~H.~Mueller and D.~Schiff,
%``Medium induced radiative energy loss: Equivalence between the BDMPS and Zakharov formalisms,''
Nucl. Phys. B \textbf{531}, 403-425 (1998)
doi:10.1016/S0550-3213(98)00546-X
[arXiv:hep-ph/9804212 [hep-ph]].
%332 citations counted in INSPIRE as of 04 Dec 2023

%\cite{Liu:2015vna}
\bibitem{Liu:2015vna}
Z.~Q.~Liu, H.~Zhang, B.~W.~Zhang and E.~Wang,
%``Quantifying jet transport properties via large $p_T$ hadron production,''
Eur. Phys. J. C \textbf{76}, no.1, 20 (2016)
doi:10.1140/epjc/s10052-016-3885-3
[arXiv:1506.02840 [nucl-th]].
%33 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Qin:2007rn}
\bibitem{Qin:2007rn}
G.~Y.~Qin, J.~Ruppert, C.~Gale, S.~Jeon, G.~D.~Moore and M.~G.~Mustafa,
%``Radiative and collisional jet energy loss in the quark-gluon plasma at RHIC,''
Phys. Rev. Lett. \textbf{100}, 072301 (2008)
doi:10.1103/PhysRevLett.100.072301
[arXiv:0710.0605 [hep-ph]].
%217 citations counted in INSPIRE as of 01 Dec 2023

%\cite{Schenke:2009gb}
\bibitem{Schenke:2009gb}
B.~Schenke, C.~Gale and S.~Jeon,
%``MARTINI: An Event generator for relativistic heavy-ion collisions,''
Phys. Rev. C \textbf{80}, 054913 (2009)
doi:10.1103/PhysRevC.80.054913
[arXiv:0909.2037 [hep-ph]].
%248 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Chen:2010te}
\bibitem{Chen:2010te}
X.~F.~Chen, C.~Greiner, E.~Wang, X.~N.~Wang and Z.~Xu,
%``Bulk matter evolution and extraction of jet transport parameter in heavy-ion collisions at RHIC,''
Phys. Rev. C \textbf{81}, 064908 (2010)
doi:10.1103/PhysRevC.81.064908
[arXiv:1002.1165 [nucl-th]].
%96 citations counted in INSPIRE as of 08 Nov 2023

%\cite{JET:2013cls}
\bibitem{JET:2013cls}
K.~M.~Burke \textit{et al.} [JET],
%``Extracting the jet transport coefficient from jet quenching in high-energy heavy-ion collisions,''
Phys. Rev. C \textbf{90}, no.1, 014909 (2014)
doi:10.1103/PhysRevC.90.014909
[arXiv:1312.5003 [nucl-th]].
%451 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Das:2015ana}
\bibitem{Das:2015ana}
S.~K.~Das, F.~Scardina, S.~Plumari and V.~Greco,
%``Toward a solution to the $R_{AA}$ and $v_2$ puzzle for heavy quarks,''
Phys. Lett. B \textbf{747}, 260-264 (2015)
doi:10.1016/j.physletb.2015.06.003
[arXiv:1502.03757 [nucl-th]].
%172 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Feal:2019xfl}
\bibitem{Feal:2019xfl}
X.~Feal, C.~A.~Salgado and R.~A.~Vazquez,
%``Jet quenching test of the QCD matter created at RHIC and the LHC needs opacity-resummed medium induced radiation,''
Phys. Lett. B \textbf{816}, 136251 (2021)
doi:10.1016/j.physletb.2021.136251
[arXiv:1911.01309 [hep-ph]].
%35 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Xie:2019oxg}
\bibitem{Xie:2019oxg}
M.~Xie, S.~Y.~Wei, G.~Y.~Qin and H.~Z.~Zhang,
%``Extracting jet transport coefficient via single hadron and dihadron productions in high-energy heavy-ion collisions,''
Eur. Phys. J. C \textbf{79}, no.7, 589 (2019)
doi:10.1140/epjc/s10052-019-7100-1
[arXiv:1901.04155 [hep-ph]].
%30 citations counted in INSPIRE as of 15 Dec 2023

%\cite{JETSCAPE:2021ehl}
\bibitem{JETSCAPE:2021ehl}
S.~Cao \textit{et al.} [JETSCAPE],
%``Determining the jet transport coefficient q̂ from inclusive hadron suppression measurements using Bayesian parameter estimation,''
Phys. Rev. C \textbf{104}, no.2, 024905 (2021)
doi:10.1103/PhysRevC.104.024905
[arXiv:2102.11337 [nucl-th]].
%109 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Xie:2022ght}
\bibitem{Xie:2022ght}
M.~Xie, W.~Ke, H.~Zhang and X.~N.~Wang,
%``Information-field-based global Bayesian inference of the jet transport coefficient,''
Phys. Rev. C \textbf{108}, no.1, L011901 (2023)
doi:10.1103/PhysRevC.108.L011901
[arXiv:2206.01340 [hep-ph]].
%25 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Xie:2022fak}
\bibitem{Xie:2022fak}
M.~Xie, W.~Ke, H.~Zhang and X.~N.~Wang,
%``Global constraint on the jet transport coefficient from single hadron, dihadron and $\gamma$-hadron spectra in high-energy heavy-ion collisions,''
[arXiv:2208.14419 [hep-ph]].
%12 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Chen:2016vem}
\bibitem{Chen:2016vem}
L.~Chen, G.~Y.~Qin, S.~Y.~Wei, B.~W.~Xiao and H.~Z.~Zhang,
%``Probing Transverse Momentum Broadening via Dihadron and Hadron-jet Angular Correlations in Relativistic Heavy-ion Collisions,''
Phys. Lett. B \textbf{773}, 672-676 (2017)
doi:10.1016/j.physletb.2017.09.031
[arXiv:1607.01932 [hep-ph]].
%78 citations counted in INSPIRE as of 29 Nov 2023

%\cite{Chen:2016cof}
\bibitem{Chen:2016cof}
L.~Chen, G.~Y.~Qin, S.~Y.~Wei, B.~W.~Xiao and H.~Z.~Zhang,
%``Dijet Asymmetry in the Resummation Improved Perturbative QCD Approach,''
Phys. Lett. B \textbf{782}, 773-778 (2018)
doi:10.1016/j.physletb.2018.06.002
[arXiv:1612.04202 [hep-ph]].
%42 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Chen:2018fqu}
\bibitem{Chen:2018fqu}
L.~Chen, G.~Y.~Qin, L.~Wang, S.~Y.~Wei, B.~W.~Xiao, H.~Z.~Zhang and Y.~Q.~Zhang,
%``Study of Isolated-photon and Jet Momentum Imbalance in $pp$ and $PbPb$ collisions,''
Nucl. Phys. B \textbf{933}, 306-319 (2018)
doi:10.1016/j.nuclphysb.2018.06.013
[arXiv:1803.10533 [hep-ph]].
%27 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Chen:2020kex}
\bibitem{Chen:2020kex}
L.~Chen, S.~Y.~Wei and H.~Z.~Zhang,
%``Probing jet medium interactions via $Z(H)$ + jet momentum imbalances,''
Eur. Phys. J. C \textbf{80}, no.12, 1136 (2020)
doi:10.1140/epjc/s10052-020-08702-4
[arXiv:2001.07606 [hep-ph]].
%5 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Zhang:2007ja}
\bibitem{Zhang:2007ja}
H.~Zhang, J.~F.~Owens, E.~Wang and X.~N.~Wang,
%``Dihadron tomography of high-energy nuclear collisions in NLO pQCD,''
Phys. Rev. Lett. \textbf{98}, 212301 (2007)
doi:10.1103/PhysRevLett.98.212301
[arXiv:nucl-th/0701045 [nucl-th]].
%212 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Zhang:2009rn}
\bibitem{Zhang:2009rn}
H.~Zhang, J.~F.~Owens, E.~Wang and X.~N.~Wang,
%``Tomography of high-energy nuclear collisions with photon-hadron correlations,''
Phys. Rev. Lett. \textbf{103}, 032302 (2009)
doi:10.1103/PhysRevLett.103.032302
[arXiv:0902.4000 [nucl-th]].
%121 citations counted in INSPIRE as of 18 Dec 2023

%\cite{Mueller:2012uf}
\bibitem{Mueller:2012uf}
A.~H.~Mueller, B.~W.~Xiao and F.~Yuan,
%``Sudakov Resummation in Small-$x$ Saturation Formalism,''
Phys. Rev. Lett. \textbf{110}, no.8, 082301 (2013)
doi:10.1103/PhysRevLett.110.082301
[arXiv:1210.5792 [hep-ph]].
%108 citations counted in INSPIRE as of 10 Dec 2023

%\cite{Mueller:2013wwa}
\bibitem{Mueller:2013wwa}
A.~H.~Mueller, B.~W.~Xiao and F.~Yuan,
%``Sudakov double logarithms resummation in hard processes in the small-x saturation formalism,''
Phys. Rev. D \textbf{88}, no.11, 114010 (2013)
doi:10.1103/PhysRevD.88.114010
[arXiv:1308.2993 [hep-ph]].
%145 citations counted in INSPIRE as of 08 Dec 2023

%\cite{Sun:2014gfa}
\bibitem{Sun:2014gfa}
P.~Sun, C.~P.~Yuan and F.~Yuan,
%``Soft Gluon Resummations in Dijet Azimuthal Angular Correlations in Hadronic Collisions,''
Phys. Rev. Lett. \textbf{113}, no.23, 232001 (2014)
doi:10.1103/PhysRevLett.113.232001
[arXiv:1405.1105 [hep-ph]].
%66 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Stasto:2018rci}
\bibitem{Stasto:2018rci}
A.~Stasto, S.~Y.~Wei, B.~W.~Xiao and F.~Yuan,
%``On the Dihadron Angular Correlations in Forward $pA$ collisions,''
Phys. Lett. B \textbf{784}, 301-306 (2018)
doi:10.1016/j.physletb.2018.08.011
[arXiv:1805.05712 [hep-ph]].
%45 citations counted in INSPIRE as of 29 Nov 2023

%\cite{Benic:2022ixp}
\bibitem{Benic:2022ixp}
S.~Beni\'c, O.~Garcia-Montero and A.~Perkov,
%``Isolated photon-hadron production in high energy pp and pA collisions at RHIC and LHC,''
Phys. Rev. D \textbf{105}, no.11, 114052 (2022)
doi:10.1103/PhysRevD.105.114052
[arXiv:2203.01685 [hep-ph]].
%14 citations counted in INSPIRE as of 12 Dec 2023

%\cite{Guo:2000nz}
\bibitem{Guo:2000nz}
X.~f.~Guo and X.~N.~Wang,
%``Multiple scattering, parton energy loss and modified fragmentation functions in deeply inelastic e A scattering,''
Phys. Rev. Lett. \textbf{85}, 3591-3594 (2000)
doi:10.1103/PhysRevLett.85.3591
[arXiv:hep-ph/0005044 [hep-ph]].
%474 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Wang:2001ifa}
\bibitem{Wang:2001ifa}
X.~N.~Wang and X.~f.~Guo,
%``Multiple parton scattering in nuclei: Parton energy loss,''
Nucl. Phys. A \textbf{696}, 788-832 (2001)
doi:10.1016/S0375-9474(01)01130-7
[arXiv:hep-ph/0102230 [hep-ph]].
%637 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Gyulassy:1990ye}
\bibitem{Gyulassy:1990ye}
M.~Gyulassy and M.~Plumer,
%``Jet Quenching in Dense Matter,''
Phys. Lett. B \textbf{243}, 432-438 (1990)
doi:10.1016/0370-2693(90)91409-5
%772 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Qin:2015srf}
\bibitem{Qin:2015srf}
G.~Y.~Qin and X.~N.~Wang,
%``Jet quenching in high-energy heavy-ion collisions,''
Int. J. Mod. Phys. E \textbf{24}, no.11, 1530014 (2015)
doi:10.1142/S0218301315300143
[arXiv:1511.00790 [hep-ph]].
%316 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Gyulassy:2000gk}
\bibitem{Gyulassy:2000gk}
M.~Gyulassy, I.~Vitev and X.~N.~Wang,
%``High p(T) azimuthal asymmetry in noncentral A+A at RHIC,''
Phys. Rev. Lett. \textbf{86}, 2537-2540 (2001)
doi:10.1103/PhysRevLett.86.2537
[arXiv:nucl-th/0012092 [nucl-th]].
%434 citations counted in INSPIRE as of 18 Dec 2023

%\cite{Wang:1998ww}
\bibitem{Wang:1998ww}
X.~N.~Wang,
%``Systematic study of high $p_{T}$ hadron spectra in $p p$, $p$ A and A A collisions from SPS to RHIC energies,''
Phys. Rev. C \textbf{61}, 064910 (2000)
doi:10.1103/PhysRevC.61.064910
[arXiv:nucl-th/9812021 [nucl-th]].
%308 citations counted in INSPIRE as of 17 Nov 2023

%\cite{Chen:2017zte}
\bibitem{Chen:2017zte}
W.~Chen, S.~Cao, T.~Luo, L.~G.~Pang and X.~N.~Wang,
%``Effects of jet-induced medium excitation in $\gamma$-hadron correlation in A+A collisions,''
Phys. Lett. B \textbf{777}, 86-90 (2018)
doi:10.1016/j.physletb.2017.12.015
[arXiv:1704.03648 [nucl-th]].
%127 citations counted in INSPIRE as of 18 Dec 2023

%\cite{Tachibana:2017syd}
\bibitem{Tachibana:2017syd}
Y.~Tachibana, N.~B.~Chang and G.~Y.~Qin,
%``Full jet in quark-gluon plasma with hydrodynamic medium response,''
Phys. Rev. C \textbf{95}, no.4, 044909 (2017)
doi:10.1103/PhysRevC.95.044909
[arXiv:1701.07951 [nucl-th]].
%124 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Tachibana:2020mtb}
\bibitem{Tachibana:2020mtb}
Y.~Tachibana, C.~Shen and A.~Majumder,
%``Bulk medium evolution has considerable effects on jet observables,''
Phys. Rev. C \textbf{106}, no.2, L021902 (2022)
doi:10.1103/PhysRevC.106.L021902
[arXiv:2001.08321 [nucl-th]].
%27 citations counted in INSPIRE as of 21 Nov 2023

%\cite{JETSCAPE:2020uew}
\bibitem{JETSCAPE:2020uew}
Y.~Tachibana \textit{et al.} [JETSCAPE],
%``Hydrodynamic response to jets with a source based on causal diffusion,''
Nucl. Phys. A \textbf{1005}, 121920 (2021)
doi:10.1016/j.nuclphysa.2020.121920
[arXiv:2002.12250 [nucl-th]].
%15 citations counted in INSPIRE as of 14 Dec 2023

%\cite{Baier:2001yt}
\bibitem{Baier:2001yt}
R.~Baier, Y.~L.~Dokshitzer, A.~H.~Mueller and D.~Schiff,
%``Quenching of hadron spectra in media,''
JHEP \textbf{09}, 033 (2001)
doi:10.1088/1126-6708/2001/09/033
[arXiv:hep-ph/0106347 [hep-ph]].
%345 citations counted in INSPIRE as of 14 Nov 2023

%\cite{Salgado:2003gb}
\bibitem{Salgado:2003gb}
C.~A.~Salgado and U.~A.~Wiedemann,
%``Calculating quenching weights,''
Phys. Rev. D \textbf{68}, 014008 (2003)
doi:10.1103/PhysRevD.68.014008
[arXiv:hep-ph/0302184 [hep-ph]].
%519 citations counted in INSPIRE as of 10 Nov 2023

%\cite{Arleo:2017ntr}
\bibitem{Arleo:2017ntr}
F.~Arleo,
%``Quenching of Hadron Spectra in Heavy Ion Collisions at the LHC,''
Phys. Rev. Lett. \textbf{119}, no.6, 062302 (2017)
doi:10.1103/PhysRevLett.119.062302
[arXiv:1703.10852 [hep-ph]].
%59 citations counted in INSPIRE as of 06 Dec 2023

%\cite{Spousta:2015fca}
\bibitem{Spousta:2015fca}
M.~Spousta and B.~Cole,
%``Interpreting single jet measurements in Pb $+$ Pb collisions at the LHC,''
Eur. Phys. J. C \textbf{76}, no.2, 50 (2016)
doi:10.1140/epjc/s10052-016-3896-0
[arXiv:1504.05169 [hep-ph]].
%85 citations counted in INSPIRE as of 06 Dec 2023

%\cite{Wang:2003mm}
\bibitem{Wang:2003mm}
X.~N.~Wang,
%``High p(T) hadron spectra, azimuthal anisotropy and back to back correlations in high-energy heavy ion collisions,''
Phys. Lett. B \textbf{595}, 165-170 (2004)
doi:10.1016/j.physletb.2004.05.021
[arXiv:nucl-th/0305010 [nucl-th]].
%194 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Hou:2019efy}
\bibitem{Hou:2019efy}
T.~J.~Hou, J.~Gao, T.~J.~Hobbs, K.~Xie, S.~Dulat, M.~Guzzi, J.~Huston, P.~Nadolsky, J.~Pumplin and C.~Schmidt, \textit{et al.}
%``New CTEQ global analysis of quantum chromodynamics with high-precision data from the LHC,''
Phys. Rev. D \textbf{103}, no.1, 014013 (2021)
doi:10.1103/PhysRevD.103.014013
[arXiv:1912.10053 [hep-ph]].
%512 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Kretzer:2000yf}
\bibitem{Kretzer:2000yf}
S.~Kretzer,
%``Fragmentation functions from flavor inclusive and flavor tagged e+ e- annihilations,''
Phys. Rev. D \textbf{62}, 054001 (2000)
doi:10.1103/PhysRevD.62.054001
[arXiv:hep-ph/0003177 [hep-ph]].
%453 citations counted in INSPIRE as of 09 Nov 2023

%\cite{Workman:2022ynf}
\bibitem{Workman:2022ynf}
R.~L.~Workman \textit{et al.} [Particle Data Group],
%``Review of Particle Physics,''
PTEP \textbf{2022}, 083C01 (2022)
doi:10.1093/ptep/ptac097
%2152 citations counted in INSPIRE as of 18 Dec 2023

%\cite{Collins:1984kg}
\bibitem{Collins:1984kg}
J.~C.~Collins, D.~E.~Soper and G.~F.~Sterman,
%``Transverse Momentum Distribution in Drell-Yan Pair and W and Z Boson Production,''
Nucl. Phys. B \textbf{250}, 199-224 (1985)
doi:10.1016/0550-3213(85)90479-1
%1525 citations counted in INSPIRE as of 16 Dec 2023

%\cite{deFlorian:2000pr}
\bibitem{deFlorian:2000pr}
D.~de Florian and M.~Grazzini,
%``Next-to-next-to-leading logarithmic corrections at small transverse momentum in hadronic collisions,''
Phys. Rev. Lett. \textbf{85}, 4678-4681 (2000)
doi:10.1103/PhysRevLett.85.4678
[arXiv:hep-ph/0008152 [hep-ph]].
%195 citations counted in INSPIRE as of 17 Nov 2023

%\cite{Catani:2000vq}
\bibitem{Catani:2000vq}
S.~Catani, D.~de Florian and M.~Grazzini,
%``Universality of nonleading logarithmic contributions in transverse momentum distributions,''
Nucl. Phys. B \textbf{596}, 299-312 (2001)
doi:10.1016/S0550-3213(00)00617-9
[arXiv:hep-ph/0008184 [hep-ph]].
%263 citations counted in INSPIRE as of 06 Dec 2023

%\cite{deFlorian:2001zd}
\bibitem{deFlorian:2001zd}
D.~de Florian and M.~Grazzini,
%``The Structure of large logarithmic corrections at small transverse momentum in hadronic collisions,''
Nucl. Phys. B \textbf{616}, 247-285 (2001)
doi:10.1016/S0550-3213(01)00460-6
[arXiv:hep-ph/0108273 [hep-ph]].
%207 citations counted in INSPIRE as of 17 Nov 2023

%\cite{Davies:1984sp}
\bibitem{Davies:1984sp}
C.~T.~H.~Davies, B.~R.~Webber and W.~J.~Stirling,
%``Drell-Yan Cross-Sections at Small Transverse Momentum,''
doi:10.1016/0550-3213(85)90402-X
%267 citations counted in INSPIRE as of 18 Dec 2023

%\cite{Ladinsky:1993zn}
\bibitem{Ladinsky:1993zn}
G.~A.~Ladinsky and C.~P.~Yuan,
%``The Nonperturbative regime in QCD resummation for gauge boson production at hadron colliders,''
Phys. Rev. D \textbf{50}, R4239 (1994)
doi:10.1103/PhysRevD.50.R4239
[arXiv:hep-ph/9311341 [hep-ph]].
%410 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Landry:2002ix}
\bibitem{Landry:2002ix}
F.~Landry, R.~Brock, P.~M.~Nadolsky and C.~P.~Yuan,
%``Tevatron Run-1 $Z$ boson data and Collins-Soper-Sterman resummation formalism,''
Phys. Rev. D \textbf{67}, 073016 (2003)
doi:10.1103/PhysRevD.67.073016
[arXiv:hep-ph/0212159 [hep-ph]].
%503 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Prokudin:2015ysa}
\bibitem{Prokudin:2015ysa}
A.~Prokudin, P.~Sun and F.~Yuan,
%``Scheme dependence and transverse momentum distribution interpretation of Collins\textendash{}Soper\textendash{}Sterman resummation,''
Phys. Lett. B \textbf{750}, 533-538 (2015)
doi:10.1016/j.physletb.2015.09.064
[arXiv:1505.05588 [hep-ph]].
%46 citations counted in INSPIRE as of 14 Dec 2023

%\cite{Sun:2014dqm}
\bibitem{Sun:2014dqm}
P.~Sun, J.~Isaacson, C.~P.~Yuan and F.~Yuan,
%``Nonperturbative functions for SIDIS and Drell\textendash{}Yan processes,''
Int. J. Mod. Phys. A \textbf{33}, no.11, 1841006 (2018)
doi:10.1142/S0217751X18410063
[arXiv:1406.3073 [hep-ph]].
%141 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Sun:2018icb}
\bibitem{Sun:2018icb}
P.~Sun, B.~Yan, C.~P.~Yuan and F.~Yuan,
%``Resummation of High Order Corrections in $Z$ Boson Plus Jet Production at the LHC,''
Phys. Rev. D \textbf{100}, no.5, 054032 (2019)
doi:10.1103/PhysRevD.100.054032
[arXiv:1810.03804 [hep-ph]].
%29 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Sun:2016kkh}
\bibitem{Sun:2016kkh}
P.~Sun, J.~Isaacson, C.~P.~Yuan and F.~Yuan,
%``Resummation of High Order Corrections in Higgs Boson Plus Jet Production at the LHC,''
Phys. Lett. B \textbf{769}, 57-61 (2017)
doi:10.1016/j.physletb.2017.02.037
[arXiv:1602.08133 [hep-ph]].
%21 citations counted in INSPIRE as of 12 Dec 2023

%\cite{Jacobs:2000wy}
\bibitem{Jacobs:2000wy}
P.~Jacobs and G.~Cooper,
%``Spatial distribution of initial interactions in high-energy collisions of heavy nuclei,''
[arXiv:nucl-ex/0008015 [nucl-ex]].
%21 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Wang:1996yf}
\bibitem{Wang:1996yf}
X.~N.~Wang,
%``pQCD based approach to parton production and equilibration in high-energy nuclear collisions,''
Phys. Rept. \textbf{280}, 287-371 (1997)
doi:10.1016/S0370-1573(96)00022-1
[arXiv:hep-ph/9605214 [hep-ph]].
%341 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Li:2001xa}
\bibitem{Li:2001xa}
S.~y.~Li and X.~N.~Wang,
%``Gluon shadowing and hadron production at RHIC,''
Phys. Lett. B \textbf{527}, 85-91 (2002)
doi:10.1016/S0370-2693(02)01179-6
[arXiv:nucl-th/0110075 [nucl-th]].
%146 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Eskola:2021nhw}
\bibitem{Eskola:2021nhw}
K.~J.~Eskola, P.~Paakkinen, H.~Paukkunen and C.~A.~Salgado,
%``EPPS21: a global QCD analysis of nuclear PDFs,''
Eur. Phys. J. C \textbf{82}, no.5, 413 (2022)
doi:10.1140/epjc/s10052-022-10359-0
[arXiv:2112.12462 [hep-ph]].
%81 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Wang:2004yv}
\bibitem{Wang:2004yv}
X.~N.~Wang,
%``Energy dependence of jet quenching and life-time of the dense matter in high-energy heavy-ion collisions,''
Phys. Rev. C \textbf{70}, 031901 (2004)
doi:10.1103/PhysRevC.70.031901
[arXiv:nucl-th/0405029 [nucl-th]].
%61 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Wang:2002ri}
\bibitem{Wang:2002ri}
E.~Wang and X.~N.~Wang,
%``Jet tomography of dense and nuclear matter,''
Phys. Rev. Lett. \textbf{89}, 162301 (2002)
doi:10.1103/PhysRevLett.89.162301
[arXiv:hep-ph/0202105 [hep-ph]].
%355 citations counted in INSPIRE as of 18 Dec 2023

%\cite{Wang:2001cs}
\bibitem{Wang:2001cs}
E.~Wang and X.~N.~Wang,
%``Parton energy loss with detailed balance,''
Phys. Rev. Lett. \textbf{87}, 142301 (2001)
doi:10.1103/PhysRevLett.87.142301
[arXiv:nucl-th/0106043 [nucl-th]].
%122 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Deng:2009ncl}
\bibitem{Deng:2009ncl}
W.~t.~Deng and X.~N.~Wang,
%``Multiple Parton Scattering in Nuclei: Modified DGLAP Evolution for Fragmentation Functions,''
Phys. Rev. C \textbf{81}, 024902 (2010)
doi:10.1103/PhysRevC.81.024902
[arXiv:0910.3403 [hep-ph]].
%92 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Pang:2012he}
\bibitem{Pang:2012he}
L.~Pang, Q.~Wang and X.~N.~Wang,
%``Effects of initial flow velocity fluctuation in event-by-event (3+1)D hydrodynamics,''
Phys. Rev. C \textbf{86}, 024911 (2012)
doi:10.1103/PhysRevC.86.024911
[arXiv:1205.5019 [nucl-th]].
%203 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Pang:2014ipa}
\bibitem{Pang:2014ipa}
L.~G.~Pang, Y.~Hatta, X.~N.~Wang and B.~W.~Xiao,
%``Analytical and numerical Gubser solutions of the second-order hydrodynamics,''
Phys. Rev. D \textbf{91}, no.7, 074027 (2015)
doi:10.1103/PhysRevD.91.074027
[arXiv:1411.7767 [hep-ph]].
%66 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Pang:2018zzo}
\bibitem{Pang:2018zzo}
L.~G.~Pang, H.~Petersen and X.~N.~Wang,
%``Pseudorapidity distribution and decorrelation of anisotropic flow within the open-computing-language implementation CLVisc hydrodynamics,''
Phys. Rev. C \textbf{97}, no.6, 064918 (2018)
doi:10.1103/PhysRevC.97.064918
[arXiv:1802.04449 [nucl-th]].
%111 citations counted in INSPIRE as of 13 Dec 2023

%\cite{Mueller:2016gko}
\bibitem{Mueller:2016gko}
A.~H.~Mueller, B.~Wu, B.~W.~Xiao and F.~Yuan,
%``Probing Transverse Momentum Broadening in Heavy Ion Collisions,''
Phys. Lett. B \textbf{763}, 208-212 (2016)
doi:10.1016/j.physletb.2016.10.037
[arXiv:1604.04250 [hep-ph]].
%65 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Mueller:2016xoc}
\bibitem{Mueller:2016xoc}
A.~H.~Mueller, B.~Wu, B.~W.~Xiao and F.~Yuan,
%``Medium Induced Transverse Momentum Broadening in Hard Processes,''
Phys. Rev. D \textbf{95}, no.3, 034007 (2017)
doi:10.1103/PhysRevD.95.034007
[arXiv:1608.07339 [hep-ph]].
%44 citations counted in INSPIRE as of 15 Dec 2023

%\cite{Majumder:2007hx}
\bibitem{Majumder:2007hx}
A.~Majumder and B.~Muller,
%``Higher twist jet broadening and classical propagation,''
Phys. Rev. C \textbf{77}, 054903 (2008)
doi:10.1103/PhysRevC.77.054903
[arXiv:0705.1147 [nucl-th]].
%82 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Qin:2012fua}
\bibitem{Qin:2012fua}
G.~Y.~Qin and A.~Majumder,
%``Parton Transport via Transverse and Longitudinal Scattering in Dense Media,''
Phys. Rev. C \textbf{87}, no.2, 024909 (2013)
doi:10.1103/PhysRevC.87.024909
[arXiv:1205.5741 [hep-ph]].
%36 citations counted in INSPIRE as of 08 Nov 2023

%\cite{Clayton:2021uuv}
\bibitem{Clayton:2021uuv}
H.~Clayton, M.~D.~Sievert and W.~A.~Horowitz,
%``Jet broadening in the opacity and twist expansions,''
Eur. Phys. J. C \textbf{82}, no.5, 437 (2022)
doi:10.1140/epjc/s10052-022-10386-x
[arXiv:2110.14737 [hep-ph]].
%7 citations counted in INSPIRE as of 29 Nov 2023

%\cite{Liou:2013qya}
\bibitem{Liou:2013qya}
T.~Liou, A.~H.~Mueller and B.~Wu,
%``Radiative $p_\bot$-broadening of high-energy quarks and gluons in QCD matter,''
Nucl. Phys. A \textbf{916}, 102-125 (2013)
doi:10.1016/j.nuclphysa.2013.08.005
[arXiv:1304.7677 [hep-ph]].
%115 citations counted in INSPIRE as of 12 Dec 2023

%\cite{Blaizot:2014bha}
\bibitem{Blaizot:2014bha}
J.~P.~Blaizot and Y.~Mehtar-Tani,
%``Renormalization of the jet-quenching parameter,''
Nucl. Phys. A \textbf{929}, 202-229 (2014)
doi:10.1016/j.nuclphysa.2014.05.018
[arXiv:1403.2323 [hep-ph]].
%104 citations counted in INSPIRE as of 15 Nov 2023

%\cite{Zakharov:2020sfx}
\bibitem{Zakharov:2020sfx}
B.~G.~Zakharov,
%``Radiative $p_{\perp }$-broadening of fast partons in an expanding quark\textendash{}gluon plasma,''
Eur. Phys. J. C \textbf{81}, no.1, 57 (2021)
doi:10.1140/epjc/s10052-021-08847-w
[arXiv:2003.10182 [hep-ph]].
%10 citations counted in INSPIRE as of 08 Nov 2023

%\cite{ATLAS:2020wmg}
\bibitem{ATLAS:2020wmg}
G.~Aad \textit{et al.} [ATLAS],
%``Medium-Induced Modification of $Z$-Tagged Charged Particle Yields in $Pb+Pb$ Collisions at 5.02 TeV with the ATLAS Detector,''
Phys. Rev. Lett. \textbf{126}, no.7, 072301 (2021)
doi:10.1103/PhysRevLett.126.072301
[arXiv:2008.09811 [nucl-ex]].
%26 citations counted in INSPIRE as of 06 Dec 2023

%\cite{CMS:2021otx}
\bibitem{CMS:2021otx}
A.~M.~Sirunyan \textit{et al.} [CMS],
%``Using Z Boson Events to Study Parton-Medium Interactions in Pb-Pb Collisions,''
Phys. Rev. Lett. \textbf{128}, no.12, 122301 (2022)
doi:10.1103/PhysRevLett.128.122301
[arXiv:2103.04377 [hep-ex]].
%26 citations counted in INSPIRE as of 18 Dec 2023

%\cite{STAR:2009ojv}
\bibitem{STAR:2009ojv}
B.~I.~Abelev \textit{et al.} [STAR],
%``Studying Parton Energy Loss in Heavy-Ion Collisions via Direct-Photon and Charged-Particle Azimuthal Correlations,''
Phys. Rev. C \textbf{82}, 034909 (2010)
doi:10.1103/PhysRevC.82.034909
[arXiv:0912.1871 [nucl-ex]].
%75 citations counted in INSPIRE as of 15 Dec 2023

%\cite{STAR:2016jdz}
\bibitem{STAR:2016jdz}
L.~Adamczyk \textit{et al.} [STAR],
%``Jet-like Correlations with Direct-Photon and Neutral-Pion Triggers at $\sqrt{s_{_{NN}}} = 200$ GeV,''
Phys. Lett. B \textbf{760}, 689-696 (2016)
doi:10.1016/j.physletb.2016.07.046
[arXiv:1604.01117 [nucl-ex]].
%73 citations counted in INSPIRE as of 18 Dec 2023

%\cite{ALICE:2020atx}
\bibitem{ALICE:2020atx}
S.~Acharya \textit{et al.} [ALICE],
%``Measurement of isolated photon-hadron correlations in $\sqrt{s_{\rm{NN}}}$ = 5.02 TeV $pp$ and $p$-Pb collisions,''
Phys. Rev. C \textbf{102}, no.4, 044908 (2020)
doi:10.1103/PhysRevC.102.044908
[arXiv:2005.14637 [nucl-ex]].
%13 citations counted in INSPIRE as of 14 Dec 2023

%\cite{Xie:2020zdb}
\bibitem{Xie:2020zdb}
M.~Xie, X.~N.~Wang and H.~Z.~Zhang,
%``$\gamma$-hadron spectra in $p$+Pb collisions at $\sqrt{s_{NN}}=$ 5.02 TeV,''
Phys. Rev. C \textbf{103}, no.3, 034911 (2021)
doi:10.1103/PhysRevC.103.034911
[arXiv:2003.02441 [hep-ph]].
%17 citations counted in INSPIRE as of 18 Dec 2023

%\cite{Jia:2019qbl}
\bibitem{Jia:2019qbl}
J.~Jia, S.~Y.~Wei, B.~W.~Xiao and F.~Yuan,
%``Medium-Induced Transverse Momentum Broadening via Forward Dijet Correlations,''
Phys. Rev. D \textbf{101}, no.9, 094008 (2020)
doi:10.1103/PhysRevD.101.094008
[arXiv:1910.05290 [hep-ph]].
%8 citations counted in INSPIRE as of 21 Nov 2023

%\cite{Wang:2016fds}
\bibitem{Wang:2016fds}
X.~N.~Wang, S.~Y.~Wei and H.~Z.~Zhang,
%``Effect of medium recoil and $p_T$ broadening on single inclusive jet suppression in high-energy heavy-ion collisions in the high-twist approach,''
Phys. Rev. C \textbf{96}, no.3, 034903 (2017)
doi:10.1103/PhysRevC.96.034903
[arXiv:1611.07211 [hep-ph]].
%18 citations counted in INSPIRE as of 12 Dec 2023
